Breaking Band: A Breakdown of High-performance Communication

The critical path of internode communication on large-scale systems is composed of multiple components. When a supercomputing application initiates the transfer of a message using a high-level communication routine such as an MPI_Send, the payload of the message traverses multiple software stacks, the I/O subsystem on both the host and target nodes, and network components such as the switch. In this paper, we analyze where, why, and how much time is spent on the critical path of communication by modeling the overall injection overhead and end-to-end latency of a system. We focus our analysis on the performance of small messages since fine-grained communication is becoming increasingly important with the growing trend of an increasing number of cores per node. The analytical models present an accurate and detailed breakdown of time spent in internode communication. We validate the models on Arm ThunderX2-based servers connected with Mellanox InfiniBand. This is the first work of this kind on Arm. Alongside our breakdown, we describe the methodology to measure the time spent in each component so that readers with access to precise CPU timers and a PCIe analyzer can measure breakdowns on systems of their interest. Such a breakdown is crucial for software developers, system architects, and researchers to guide their optimization efforts. As researchers ourselves, we use the breakdown to simulate the impacts and discuss the likelihoods of a set of optimizations that target the bottlenecks in today's high-performance communication.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=main

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}


%.pdf: $(PACKAGE).tex
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<


%.cls:   %.ins %.dtx
	pdflatex $<




.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut main.pdf

distclean: clean

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> text/definitions.tex <==
\subsection{Definitions}
\label{sec:definitions}

Below, we define keywords to denote the time spent in each of
the components involved in initiating and transmitting a
message.

\begin{itemize}
	\item \post -- time spent by the CPU to perform a PIO post. This
	includes the time to prepare the message descriptor and copying
	it into the memory-mapped location of the NIC's memory.
	\item \poll -- time spent by the CPU to perform one poll operation
	on the completion queue. 
	\item \pcie -- time spent on the PCIe subsystem when the message
	payload traverses from the node to the NIC, that is, from the RC
	to the NIC.
	\fix{\item \wire -- time spent on the interconnect's wire between two
		NICs.} % depends on how I present the switch latency numbers; might need to add another switch category
	\item \rctomem[x] -- time spent in writing an \emph{x} byte payload
	from the RC to memory.
\end{itemize}
